Performance of Distribution Regression with Doubling Measure under the seek of Closest Point

We study the distribution regression problem assuming the distribution of distributions has a doubling measure larger than one. First, we explore the geometry of any distributions that has doubling measure larger than one and build a small theory around it. Then, we show how to utilize this theory to find one of the nearest distributions adaptively and compute the regression value based on these distributions. Finally, we provide the accuracy of the suggested method here and provide the theoretical analysis for it.

==> README <==

March 5, 2007


IEEEtran is the official LaTeX class for authors of the Institute of
Electrical and Electronics Engineers (IEEE) transactions journals and
conferences. The latest version of the IEEEtran package can be found
at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/


Version 1.7a is a bug fix release that corrects the two column peer
review title page problem. This problem was not present in the 1.6 series.


V1.7 is a significant update over the 1.6 series with many important
changes. For a full list, please read the file changelog.txt. The most
notable changes include:

 1. New class option compsoc to support the IEEE Computer Society format.

 2. Several commands and environments have been deprecated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow the use of
    the obsolete forms (for now), but with a warning message to the console
    during compilation:
    \IEEEauthorblockA, \IEEEauthorblockN, \IEEEauthorrefmark,
    \IEEEbiography, \IEEEbiographynophoto, \IEEEkeywords, \IEEEPARstart,
    \IEEEproof, \IEEEpubid, \IEEEpubidadjcol, \IEEEQED, \IEEEQEDclosed,
    \IEEEQEDopen, \IEEEspecialpapernotice. IEEEtran.cls now redefines
    \proof in way to avoid problems with the amsthm.sty package.
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
    These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. New \CLASSINPUT, \CLASSOPTION and \CLASSINFO interface allows for more
    user control and conditional compilation.

 4. Several bug fixes and improved compatibility with other packages.


A note to those who create classes derived from IEEEtran.cls: Consider the
use of patch code, either in an example .tex file or as a .sty file,
rather than creating a new class. The IEEEtran.cls CLASSINPUT interface
allows IEEEtran.cls to be fully programmable with respect to document
margins, so there is no need for new class files just for altered margins.
In this way, authors can benefit from updates to IEEEtran.cls and the need
to maintain derivative classes and backport later IEEEtran.cls revisions
thereto is avoided. As always, developers who create classes derived from
IEEEtran.cls should use a different name for the derived class, so that it
cannot be confused with the official/base version here, as well as provide
authors with technical support for the derived class. It is generally a bad
idea to produce a new class that is not going to be maintained.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for conference papers.

bare_jrnl.tex          - A bare bones starter file for journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_jrnl.tex, bare_jrnl_compsoc.tex
***************************************************************************


==> conclusion.tex <==
\section{Conclusion}

Finally here we are discussing the conclusion of the work of this paper

==> proof.tex <==
\begin{theorem} 
Assume $\Psi$ is a distribution which has doubling dimension of $d$ and $s$ be a fixed point that is sampled from the distribution.
Given that, $\Omega$ is a set of $m$ points those are sampled from $\Psi$, then we can claim the expected distance of $s$ to $\Omega$ is bounded by $m^{-\frac{1}{d}}$ asymptotically:
\begin{align*}
    \EX \big[ \mathrm{min}\{ \| s-\omega \| | \omega \in \Omega \} \big] \in \mathcal{O}\big(m^{-\frac{1}{d}}\big)
\end{align*}
\end{theorem}
\begin{proof} Given that $\Psi$ is a distribution that has a doubling dimension, then from the definition, we have
\begin{align*}
  \frac{\mathbb{P}(B(s, r))}{ \mathbb{P}(B(s,\epsilon r))} \leq (\frac{1}{\epsilon})^d   
\end{align*}
Picking $r=1$ and $\epsilon = \frac{1}{2^i}$ results 
\begin{align*}
  \frac{\mathbb{P}(B(s, 1))}{ \mathbb{P}(B(s,\frac{1}{2^i} ))} \leq 2^{id}   
\end{align*}
Using the fact $\mathbb{P}(B(s,1 )) = 1$ and algebraic manipulations, we conclude:
\begin{align}
  \mathbb{P} \Big(B(s,\frac{1}{2^i} )\Big) \geq \frac{1}{2^{id}}   
\end{align}
Then using (1) we can make following 3 conclusions:\\
\begin{itemize}
    \item  If $\Omega$ is a set that contains just one point, then the probability of distance of this point to $s$  being in the interval $[0, \frac{1}{2^i}]$ is at least $\frac{1}{2^{id}}$ 
    \item  If $\Omega$ is a set that contains just one point, then the probability of distance of this point to $s$  being in the interval $[\frac{1}{2^i}, 1]$ is at most $1-\frac{1}{2^{id}}$  
    \item  If $\Omega$ is a set that contains $m$ points, then the probability of minimum distance from $s$ to $\Omega$ being in the interval $[\frac{1}{2^i}, 1]$ is at most $\big(1-\frac{1}{2^{id}}\big)^m$ \\ 
\end{itemize}
Basically, the first conclusion is restatement of inequality (1), the second conclusion is just the completion of the first one using $\mathbb{P}(B(s,1))=1$. 
The last conclusion is due to independence of points of $\Omega$.
Using these conclusions, we obtain the following inequality:
\begin{align*}
 \EX [min\{ \| &s -\omega \| | \omega \in \Omega \}]   \\
                        &\leq  1* \mathbb{P} \Big( \mathrm{min}\{ \| s- \omega \| | \omega \in \Omega \} > \frac{1}{2} \Big)     \\
                        &\:\:\:\: +\frac{1}{2}* \mathbb{P} \Big(\frac{1}{2} \geq \mathrm{min}\{ \| s-\omega\| | \omega \in \Omega \} > \frac{1}{4} \Big)  \\
                        &\:\:\:\: +\frac{1}{4}* \mathbb{P}\Big(\frac{1}{4} \geq \mathrm{min} \{ \| s-\omega\| | \omega \in \Omega \} > \frac{1}{8} \Big)  \\
                        &\:\:\:\:\:\:\:\: \vdots \\
                        &\leq  1* \Big( \big[1- \frac{1}{2^d}\big]^m -\big[1-\frac{1}{2^0}\big]^m  \Big) \\
                        &\:\:\:\: + \frac{1}{2^{1}}* \Big( \big[1-\frac{1}{2^{2d} }\big]^m -\big[1- \frac{1}{2^d }\big]^m  \Big)  \\          
                        &\:\:\:\: + \frac{1}{2^{2}}* \Big( \big[1-\frac{1}{2^{3d} }\big]^m -\big[1-\frac{1}{2^{2d} }\big]^m  \Big)  \\
                        &\:\:\:\:\:\:\:\: \vdots 
\end{align*}
The first inequality is due to the observation if $t$ is a random variable from the interval $[0,1]$, then 
\begin{align*}
    \mathbb{E}[t] = \mathbb{P}(t>\frac{1}{2}) &+ \frac{1}{2} \mathbb{P}(\frac{1}{4}<t \leq \frac{1}{2}) \\
                                              &+ \frac{1}{2^2} \mathbb{P}(\frac{1}{2^3}<t \leq \frac{1}{2^2}) \\
                                              & \vdots
\end{align*}
no matter what underlying distribution is, and the second inequality is due to lemma below:
\begin{lemma} Given $s$ is a fixed point sampled from $\Psi$, and also $\Omega$ is the set of $m$ independent points sampled the same distribution. Then, the following inequality get satisfied:
\begin{align*}
 \sum_{i=0}^{\infty} \frac{1}{2^i} \mathbb{P}\Big(\frac{1}{2^i} &\geq \mathrm{min}\{ \| s-\omega \| | \omega \in \Omega \} > \frac{1}{2^{i+1}} \Big) \\ 
 &\leq \sum_{i=0}^{\infty} \frac{1}{2^i}  \Big( \Big[1-\frac{1}{2^{(i+1)d}}\big]^m - \big[1-\frac{1}{2^{id}}\big]^m  \Big)     
\end{align*}
\end{lemma}
we prove this lemma at the end of the proof of the theorem.
Returning back to the bound:
\begin{align*}
 \EX [min\{ \| s &-\omega \| | \omega \in \Omega \}]   \\
                &\leq  \sum_{i=0} \frac{1}{2^i} \Big( \big[1- \frac{1}{2^{id}} \big]^m - \big[1- \frac{1}{2^{(i-1)d}} \big]^m \Big)
\end{align*}
In the remaining of the proof, we show that the summation above is bounded by $\mathcal{O}(m^{-1/d})$, which is sufficient for the statement of the theorem.
To prove the bound for the summation, we are splitting the infinite sum into two and show both parts are bounded by $\mathcal{O}(m^{-1/d})$ which implies their sum is also bounded by $\mathcal{O}(m^{-1/d})$.
\begin{align*}
    \sum_{i=0} &\frac{1}{2^i} \Big( \big[1 - \frac{1}{2^{id}} \big]^m - \big[1- \frac{1}{2^{(i-1)d}} \big]^m \Big) \\
    &= \sum_{i=0}^{ \floor{\frac{\log{m} }{d} } } \frac{1}{2^i} \Big( \big[1- \frac{1}{2^{id}} \big]^m - \big[1- \frac{1}{2^{(i-1)d}} \big]^m \Big)  \\
    &\:\:+\sum_{ \floor{i=\frac{\log{m}}{d} }+1 } \frac{1}{2^i} \Big( \big[1- \frac{1}{2^{id}} \big]^m - \big[1- \frac{1}{2^{(i-1)d}} \big]^m \Big)  \\
    &\leq \sum_{i=0}^{ \floor{ \frac{\log{m}}{d}  } } \frac{1}{2^i} \Big( \big[1- \frac{1}{2^{id}} \big]^m - \big[1- \frac{1}{2^{(i-1)d}} \big]^m \Big)  \\
    &\:\:+\frac{1}{2^{ \floor{ \frac{\log{m}}{d}}+1}} \sum_{i= \floor{\frac{\log{m}}{d} } +1 } \Big( \big[1- \frac{1}{2^{id}} \big]^m - \big[1- \frac{1}{2^{(i-1)d}} \big]^m \Big)   \\
    &\leq \sum_{i=0}^{ \floor{ \frac{\log{m}}{d}  } } \frac{1}{2^i} \Big( \big[1- \frac{1}{2^{id}} \big]^m - \big[1- \frac{1}{2^{(i-1)d}} \big]^m \Big)  + \frac{1}{2^{  \frac{\log{m}}{d}}}     \\
    &= \sum_{i=0}^{ \floor{ \frac{\log{m}}{d}  } } \frac{1}{2^i} \Big( \big[1- \frac{1}{2^{id}} \big]^m - \big[1- \frac{1}{2^{(i-1)d}} \big]^m \Big)  + m^{-1/d}      
\end{align*}
The first inequality is due to if $i\geq \floor{ \frac{\log{m}}{d}}+1$ then we have $ \frac{1}{2^i} \leq \frac{1}{2^{ \floor{ \frac{\log{m}}{d}}+1}}$ also true. 
For the second inequality, we used $\floor{ \frac{\log{m}}{d}  }+ 1 \geq \frac{\log{m}}{d}$ and 
\begin{align*}
 \sum_{i= \floor{\frac{\log{m}}{d} } +1 } \Big( \big[1- \frac{1}{2^{id}} \big]^m - \big[1- \frac{1}{2^{(i-1)d}} \big]^m \Big) \leq 1   
\end{align*}
due to telescopic sum argument.
Hence, we have:
\begin{align*}
 \EX [\mathrm{min} &\{ \| s -\omega \| | \omega \in \Omega \}]   \\
                &\leq  \sum_{i=0}^{ \floor{ \frac{\log{m}}{d}  } } \frac{1}{2^i} \Big( \big[1- \frac{1}{2^{id}} \big]^m - \big[1- \frac{1}{2^{(i-1)d}} \big]^m \Big)  + m^{-\frac{1}{d}}  
\end{align*}
All we should do in the rest of the proof, is to show the first summand is also bounded by $\mathcal{O}(m^{-1/d})$.
\begin{align*}
  \sum_{i=0}^{ \floor{ \frac{\log{m}}{d}  } } \frac{1}{2^i} \Big( \big[1- \frac{1}{2^{id}} \big]^m &- \big[1- \frac{1}{2^{(i-1)d}} \big]^m \Big)  \\
   &\leq   \sum_{i=0}^{ \floor{ \frac{\log{m}}{d}  } } \frac{1}{2^i}  \big[1- \frac{1}{2^{id}} \big]^m   \\
   &\leq   \sum_{i=0}^{ \floor{ \frac{\log{m}}{d}  } } \frac{1}{2^i} e^ {- \frac{m}{2^{id}} }     
\end{align*}
To bound the latest sum, we will use the fact that 
\begin{align*}
 \sum_{i=1}^{k} x_i \leq x_k (1+1/\alpha + 1/\alpha^2 + \ldots)   
\end{align*}
get satisfied if for any $i\leq k$ the ratio $\frac{x_i}{x_{i-1}} \geq \alpha$ has lower bound $\alpha$.
In this case, we show that for $\alpha = \frac{e}{2}$ we have the ration lower bounded as below:
\begin{align*}
\frac{   \frac{1}{2^i} e^ {- \frac{m}{2^{id}} }  }{   \frac{1}{2^{i-1}} e^{- \frac{m}{2^{(i-1)d}} } } = \frac{1}{2} e^{  \frac{m}{2^{id}}  (2^d-1)} \geq \frac{e}{2}
\end{align*}
where we used, $d\geq 1$ and $i \leq \frac{\log{m}}{d}$ implies $2^d-1\geq 1$ and $e^{\frac{m}{2^{id}}} \geq e $. 
Returning back to the summation above:
\begin{align*}
    \sum_{i=0}^{ \floor{ \frac{\log{m}}{d}  } } \frac{1}{2^i} e^ {- \frac{m}{2^{id}} }   &\leq   \frac{1}{2^{ \floor{ \frac{\log{m}}{d}  } }}  e^ {- \frac{m}{2^{\floor{ \frac{\log{m}}{d}  }d}} } \big( 1 + \frac{2}{e} + (\frac{2}{e})^2 + \ldots \big)\\
&\leq   \frac{1}{2^{ \floor{ \frac{\log{m}}{d}  } }}  e^ {-1 } \frac{1}{1-2/e} \\
&\leq   \frac{2}{2^{  \frac{\log{m}}{d}  }}  e^ {-1 } \frac{1}{1-2/e} = 2 m^{-\frac{1}{d}} \frac{1}{e-2}\\
\end{align*}
Therefore, putting it all together, we conclude that\\
\begin{align*}
 \EX [\mathrm{min} &\{ \| s -\omega \| | \omega \in \Omega \}]    \leq  \frac{2}{e-2}  m^{-\frac{1}{d}}  + m^{-\frac{1}{d}}  
\end{align*}
as desired.
\end{proof}


\begin{proof}[proof of lemma 1]
As we mentioned in the previous proof the probability of all points being in larger distance than $\frac{1}{2}$ is at most $(1-\frac{1}{2^d})^m$. 
Note that the event of all points having distance that is larger than $\frac{1}{2}$ is equivalent to the event of minimum being distant larger than $\frac{1}{2}$
Therefore, we can write it as:
\begin{align*}
     \mathbb{P}( \mathrm{min}\{ \| s-\omega \| | \omega \in \Omega \} > \frac{1}{2^{1}})< \big[1-\frac{1}{2^d}\big]^m    
\end{align*}
Using the fact that $\mathbb{P}(B(s,1))=1$, we can see that 
\begin{align*}
 \mathbb{P}( \mathrm{min}\{ \| s&-\omega \| | \omega \in \Omega \} > \frac{1}{2^{1}}) \\
 &= \mathbb{P}(\frac{1}{2^0} > \mathrm{min}\{ \| s-\omega \| | \omega \in \Omega  \} > \frac{1}{2^{1}})
\end{align*}
Observing the equation of $1-\frac{1}{2^0} = 0$ we conclude :
\begin{align*}
 \mathbb{P}(\frac{1}{2^0} > \mathrm{min}\{ \| s&-\omega \| | \omega \in \Omega \} > \frac{1}{2^{1}}) \\
 &\leq   \Big( \big[1-\frac{1}{2^{d}}\big]^m -\big[1-\frac{1}{2^0}\big]^m  \Big) 
\end{align*}
Next step is to argue similar statement for general $i$.
The probability of all points being larger distance than $\frac{1}{2^i}$ is at most $\big[1-\frac{1}{2^{id}}\big]^m$.  
Similar as above, this statement is equivalent to:
\begin{align*}
    \mathbb{P}( \mathrm{min}\{ \| s-\omega \| | \omega \in \Omega \} > \frac{1}{2^{i}})< \big[1- \frac{1}{2^{id}}\big]^m
\end{align*}
Note that:
\begin{align*}
     \mathbb{P}( \mathrm{min}\{ \| &s-\omega\| | \omega \in \Omega \} > \frac{1}{2^{i}}) \\ 
     &=   \mathbb{P}(\frac{1}{2^0} \geq  \mathrm{min}\{ \| s-\omega \| | \omega \in \Omega \} > \frac{1}{2^{i}})  \\
     &=  \mathbb{P}(\frac{1}{2^{i-1}} \geq  \mathrm{min}\{ \| s- \omega \| | \omega \in \Omega \} > \frac{1}{2^{i}})  \\
     &\:\:+  \mathbb{P}(\frac{1}{2^{i-2}} \geq  \mathrm{min}\{ \| s-\omega \| | \omega \in \Omega \} > \frac{1}{2^{i-1}})  \\
     &\:\:+  \mathbb{P}(\frac{1}{2^{i-3}} \geq  \mathrm{min}\{ \| s-\omega \| | \omega \in \Omega \} > \frac{1}{2^{i-2}})  \\
     &\:\:\vdots  \\
     &\:\:+  \mathbb{P}(\frac{1}{2^{0}} \geq  \mathrm{min}\{ \| s-\omega \| | \omega \in \Omega \} > \frac{1}{2^{1}})
\end{align*}
One can observe from the telescopic sum argument following is true:
\begin{align*}
  \big[1-\frac{1}{2^{id}}\big]^m &= \big[1-\frac{1}{2^{id}}\big]^m -\big[1-\frac{1}{2^0}\big]^m      \\
                        &=\big[1-\frac{1}{2^{id}}\big]^m -\big[1-\frac{1}{2^{(i-1)d}}\big]^m     \\
                        &\:\:\:+\big[1-\frac{1}{2^{(i-1)d}}d\big]^m -\big[1-\frac{1}{2^{(i-2)d}}\big]^m \\
                        &\:\:\:\vdots                                                    \\
                        &\:\:\:+\big[1-\frac{1}{2^{d}}\big]^m -\big[1-\frac{1}{2^{0}}\big]^m 
\end{align*}
Therefore, the inequality above is equivalent to:
\begin{align*}
   \sum_{j=0}^{i}  \mathbb{P}\Big(\frac{1}{2^j} > \mathrm{min}\{ &\| s- \omega \| | \omega \in \Omega \} > \frac{1}{2^{j+1}} \Big)   \\  
    &\leq  \sum_{j=0}^{i}   \Big( \big[1-\frac{1}{2^{(j+1)d}}\big]^m - \big[1-\frac{1}{2^{jd}}\big]^m  \Big) 
\end{align*}
Multiplying both side of the inequality by $\frac{1}{2^j}$ conclude for any $i$ following inequality to be satisfied:
\begin{align*}
   \sum_{j=0}^{i}  \frac{1}{2^{i+1}} \mathbb{P}\Big(\frac{1}{2^j} > \mathrm{min}\{ \| s-\omega \| | \omega \in \Omega \} > \frac{1}{2^{j+1}} \Big)     \\
    \leq \sum_{j=0}^{i}   \frac{1}{2^{i+1}} \Big( \big[1-\frac{1}{2^{(j+1)d}}\big]^m -\big[1-\frac{1}{2^{jd}} \big]^m  \Big) 
\end{align*}
Summing both side of the equation with respect to results with the following inequality:
\begin{align*}
  \sum_{i=0}^{\infty} \sum_{j=0}^{i}  \frac{1}{2^{i+1}} \mathbb{P}\Big(\frac{1}{2^j} > \mathrm{min}\{ \| s-\omega\| | \omega \in \Omega \} > \frac{1}{2^{j+1}} \Big)  \\  
  \leq  \sum_{i=0}^{\infty} \sum_{j=0}^{i}   \frac{1}{2^{i+1}} \Big( \big[1-\frac{1}{2^{(j+1)d}}\big]^m -\big[1-\frac{1}{2^{jd}}\big]^m  \Big) 
\end{align*}
Reversing the order of the variables in the sum we get:
\begin{align*}
\sum_{j=0}^{\infty} \sum_{i=j}^{\infty}  \frac{1}{2^{i+1}} \mathbb{P}\Big(\frac{1}{2^j} > \mathrm{min}\{ \| s-\omega \| | \omega\in \Omega \} > \frac{1}{2^{j+1}} \Big) \\
\leq   \sum_{i=0}^{\infty} \sum_{i=j}^{\infty}   \frac{1}{2^{i+1}} \Big( \big[1-\frac{1}{2^{(j+1)d}}\big]^m -\big[1-\frac{1}{2^{jd}}\big]^m  \Big) 
\end{align*}
We can see the right multiplication for each side of the inequality is constant with respect to $j$ which allows us to write summation in the form of:
\begin{align*}
  \sum_{j=0}^{\infty}  \mathbb{P}\Big(\frac{1}{2^j} > \mathrm{min}\{ \| s-\omega \| | \omega \in \Omega \} > \frac{1}{2^{j+1}} \Big)  \sum_{i=j}^{\infty}   \frac{1}{2^{i+1}}   \\
  \leq   \sum_{j=0}^{\infty} \Big( \big[1-\frac{1}{2^{(j+1)d}} \big]^m -\big[1-\frac{1}{2^{jd}}\big]^m  \Big) \sum_{i=j}^{\infty}   \frac{1}{2^{i+1}}  
\end{align*}
by replacing $\sum_{i=j}^{\infty} \frac{1}{2^{i+1}}$ with $\frac{1}{2^i}$ we get:
\begin{align*}
  \sum_{j=0}^{\infty}  \mathbb{P}\Big(\frac{1}{2^j} > \mathrm{min}\{ \| s-\omega \| | \omega \in \Omega \} > \frac{1}{2^{j+1}} \Big)  \frac{1}{2^{j+1}}  \\  
   \leq \sum_{i=0}^{\infty} \Big( \big[1-\frac{1}{2^{(j+1)d}}\big]^m - \big[1-\frac{1}{2^{jd}}\big]^m  \Big) \frac{1}{2^{j}}  
\end{align*}
which is equivalent to lemma statement:
\begin{align*}
   \sum_{i=0}^{\infty} \frac{1}{2^i} \mathbb{P}\Big(\frac{1}{2^i} > \mathrm{min}\{ \| s-\omega \| | \omega \in \Omega \}  > \frac{1}{2^{i+1}}\Big)  \\
   \leq \sum_{i=0}^{\infty} \frac{1}{2^i}  \Big( \big[1-\frac{1}{2^{(i+1)d}}\big]^m -\big[1-\frac{1}{2^{id}}\big]^m  \Big)  
\end{align*}

\end{proof}

%We can claim summation after this term is also $\Theta(\frac{1}{m^{1/d}} \log{m})$.
%Lets find the point where  $(\frac{1}{2^{k}})^d = \frac{\log{m}}{m}$ satisfies.
%This will happen when $k = (\frac{m}{\log{m}})^{1/d}$ and
%$1-(\frac{1}{2^{k}})^d = 1 - \frac{\log{m}}{m}$ will also be true here.
%Therefore,
%$(1-(\frac{1}{2^{k}})^d )^m < (1 - \frac{\log{m}}{m})^m = (\frac{1}{e})^{\log{m}}=
%\frac{1}{m}$.

%Simply upper bounding all the powers of two here by 1 and upper bounding left element of parenthesis by 1 we can claim after this $k$ to the previously selected $k$ summation is upper bounded by $\frac{1/d \log{m}}{m}$.

%Additionally, for the terms before this selected $k$, we can simply upper bound powers of two's by $\frac{\log{m}}{m}$ and telescopic sum inside paranthesis is upper bounded by 1 therefore entire sum is upper bounded by $\frac{\log{m}}{m}$.
 
%At the end, if we just sum these three numbers we can see :

%$$\frac{1}{m^{1/d}} + \frac{1/d \log{m}}{m} + \frac{\log{m}}{m}$$

%which is upper bounded by the first summand under the constraint $d > 1$.


